Retrieve, Caption, Generate: Visual Grounding for Enhancing Commonsense in Text Generation Models

We investigate the use of multimodal information contained in images as an effective method for enhancing the commonsense of Transformer models for text generation. We perform experiments using BART and T5 on concept-to-text generation, specifically the task of generative commonsense reasoning, or CommonGen. We call our approach VisCTG: Visually Grounded Concept-to-Text Generation. VisCTG involves captioning images representing appropriate everyday scenarios, and using these captions to enrich and steer the generation process. Comprehensive evaluation and analysis demonstrate that VisCTG noticeably improves model performance while successfully addressing several issues of the baseline generations, including poor commonsense, fluency, and specificity.

==> sections/TODOS_for_AAAI_and_Cam-Ready.tex <==
-Combine content into a single .tex file
-CUT DOWN TO 7 PAGES BODY!
-Go through AAAI cam-ready instructions and ensure no issues


DONE:
-MAYBE IMPROVE TITLE, e.g. "retrieve, caption, generate"? for AAAI
-MAYBE ADD LEARNING RATES AND OTHER TRAINING + GENERATION MODEL DETAILS FOR AAAI
-IMPROVE HUMAN EVAL AND ALSO GET GOOD STAT SIG AND IAA VALUES FOR AAAI

FORGET IT:
-MAYBE IMPROVE ABSTRACT (NOT AS ABRUPT START) FOR AAAI
-MAYBE IMPROVE TABLES (E.G. USING BOOKTABS) FOR AAAI
-ADD MORE AAAI CITATIONS [OR REPLACE EQUIVALENTS WITH AAAI counterparts]
-MAYBE ADD MORE EXAMPLES OF IMAGES AND CAPTIONS FOR AAAI

CAM-READY FINISHED:
-Add link to GitHub repo
-Fix references/links between sections and stuff in the rendered PDF
-IMPORTANT!!! DELETE THE NINESIZE OPTION ADDED TO AAAI22.STY FOR SMALLER FONT SIZE. and also change \ninesize to \small for all (or at least most) tables and captions. (wasn't necessary since this was only used for NAREOR)
-Add self-citations (survey, GenAug, NAREOR, ALOHA, SAPPHIRE, SMERTI, etc.)
-Cite and compare to SAPPHIRE models for CAM-READY

==> sections/abstract_backup.tex <==
We investigate the use of multimodal information contained in images as an effective improvement for concept-to-text natural language generation. We call this approach VisCTG: Visually-Grounded Concept-to-Text Generation. We illustrate VisCTG's effectiveness using BART and T5 models on the task of generative commonsense reasoning, or \emph{CommonGen}. VisCTG involves captioning images representing appropriate everyday scenarios, and using these captions to enrich and steer the generation process. Comprehensive evaluation demonstrates that VisCTG improves model performance to a noticeable degree. Detailed qualitative analysis shows that VisCTG successfully addresses several issues of the baseline generations, including insufficient commonsense, poor fluency, and inadequate specificity.% while having potential for further exploration and application to general constrained text generation and NLG tasks.
%\sy{Set Augmentation and Post-hoc PHrase Infilling and REcombination}
%  of varying sizes - unncessary : vg
%MAYBE IMPROVE ABSTRACT (NOT AS ABRUPT START) FOR AAAI

==> sections/conclusion_backup.tex <==
\vspace{-2mm}
In conclusion, we motivated and investigated the use of visual-grounding for concept-to-text generation which we call VisCTG: Visually-Grounded Concept-to-Text Generation. Extensive experiments on BART and T5 showed its effectiveness on the CommonGen task. Comprehensive evaluation demonstrated that VisCTG improves model performance while addressing several issues of the baselines, and has potential for further exploration. Potential future work includes improving the image search and captioning, e.g. a method to select better images during scraping, using a stronger captioning model, or first finetuning it on a subset of CommonGen. VisCTG can be investigated for other data-to-text NLG tasks, e.g. WebNLG. Video captioning and image generation rather than scraping can also be explored. %Leveraging the CLIP representation \cite{radford2021learning}, which can embed arbitrary text inputs into image space, could be another route to generalize via the visual modality starting from text.

%\vg{Another formulation to explore could be incorporating off-the-shelf text-to-image generators into our pipeline, which might open complementary generalization pathways to retrieve-and-caption.}
%\vg{x} 

%video captioning. or improving the image search somehow to actually skip images on the spot that are not suitable or using a better corpus rather than simply google search (although this is kind of slapping ourselves because then reviewers will be like "why didn't u do that in the first place?"). or improving the captioning model by finetuning it on subset of commongen data first


%They can also be explored for applications such as paraphrase generation, grammatical error correction, and data augmentation \cite{feng2021survey}. %, particularly for text generation \cite{feng-etal-2020-genaug}. Removed by vg - irreleavnt nd too much of a stretch

%Generalizing methods devised here on related, semi to mildly structured data-to-text NLG tasks, such as WebNLG \cite{gardent2017webnlg} could be a promising extension. 

%\sy{Need to discuss future work: one direction is improving BART-MI, not sure about others. Need to discuss with Varun about more future directions. Maybe use our methods (e.g. phrase recombo) for data augmentation as it generates paraphrases? Investigate it for other tasks like GEC too. Of course, explicitly investigate them for other constrained sentence generation tasks and data-to-text NLG tasks. Maybe also mention that the methods can possibly be improved with further training data (e.g. phrase recombo is essentially a "more difficult" version of key-to-text and may require more training data to become even more effective). Maybe also investigate other things such as concept set order permutation, keyword replacement, etc. Also, loss function improvements for improving coverage and stuff, try sampling other than beam search for diversity + fluency, keyword augmentation using KGs like ConceptNet, maybe combination of our approaches (e.g. kw-aug + att-aug or either one combined with phrase recombo)}
%\sy{BTW, no need for ethics statement right?}
%\sy{Also, make decision later about whether to submit code and data}
%\vg{"Maybe also mention that the methods can possibly be improved with further training data" - I think that's an obvious thing for most methods right}

%\vg{ Generalizing methods devised here on related, semi to mildly structured data-to-text NLG tasks, such as WebNLG \cite{gardent2017webnlg} could be a promising extension. Better exploiting other regularities natural to Commongen-like tasks, such as invariance to input order permutation presents another avenue.}

%\sy{FIND A WAY TO CITE SAPPHIRE, SURVEY PAPER, GENAUG, ETC. FOR CAM-READY?}

==> sections/intro_backup.tex <==
Constrained text generation and data-to-text natural language generation (NLG) are areas in NLP research that have seen increasing interest. They involve generating natural language outputs given certain pre-conditions, e.g. specific words in the outputs, and structured or semi-structured inputs, respectively. Their task formulation typically involves converting a set of inputs into natural language text. These inputs can normally be thought of as \textit{concepts}, or high-level words or structures, that play an important role in the generated text.

Transformer-based models have seen increasing popularity and application to several NLP tasks. Model improvements such as larger and better pretrained language generation models is a large reason for performance gains. However, are there effective improvements that can come from the use of information from other modalities such as vision?

In this paper, we propose an effective improvement for concept-to-text generation called VisCTG: Visually-Grounded Concept-to-Text Generation. VisCTG involves captioning images that effectively and logically represent the input concepts, and using these captions to guide and enhance the final generation process. See Table \ref{tab:image_caption_examples} for examples. Multimodal work has become increasingly popular in ML and NLP, but its investigation for constrained and data-to-text NLG has been limited \cite{multimodal_survey_1,multimodal_survey_2}.\footnote{All code and data will be released upon acceptance.}%,multimodal_survey_3,multimodal_survey_4}.

\begin{table*}[t]
\centering
\small
\resizebox{\columnwidth}{!}{\begin{tabular}{ |c|c| } 
 \hline
 \textit{\{stand, hold, umbrella, street\}} & \textit{\{field, player, team, walk\}}\\
 \includegraphics[width=0.35\textwidth]{images/example_img_1.jpg} & \raisebox{1pt}{\includegraphics[width=0.40\textwidth]{images/example_img_2.jpg}}\\
 \textbf{capt:} a woman walking down a street holding an umbrella & \textbf{capt:} a group of baseball players standing on a field\\
 \textbf{gen:} A woman stands on a street holding an umbrella. & \textbf{gen:} players walk onto the field during the match \\& between football teams.\\[0.5mm]
 \hline%\\[-2ex]
 \rule{0pt}{0.9\normalbaselineskip}
 \textit{\{cat, bed, pet, lay\}} & \textit{\{fence, jump, horse, rider\}}\\
 \includegraphics[width=0.25\textwidth]{images/example_img_3.png} & \raisebox{1pt}{\includegraphics[width=0.35\textwidth]{images/example_img_4.jpg}}\\
 \textbf{capt:} a cat laying on a bed with a stuffed animal & \textbf{capt:} a horse is jumping over a wooden fence\\
 \textbf{gen:} A cat laying on a bed being petted. & \textbf{gen:} A rider jumps a fence on a horse.\\
  \hline
\end{tabular}}
\vspace{-2mm}
\caption{Examples of retrieved images for select input concept sets. Corresponding captions and final generations are below the images.}%\sy{associated final outputs with each example: 1. A woman stands on a street holding an umbrella. (T5-large seed1), 2. players walk onto the field during the match between football teams. (T5-large seed1), 3. A cat laying on a bed being petted. (BART-large seed1), 4. A rider jumps a fence on a horse. (T5-large seed1)}}
\label{tab:image_caption_examples}
\vspace{-5mm}
\end{table*}

We investigate the task of generative commonsense reasoning, or CommonGen \cite{lin-etal-2020-commongen}, which involves generating sentences that effectively describe everyday scenarios from concepts sets, or words that must appear in the output in some form. CommonGen is challenging as effective relational reasoning ability using commonsense knowledge is required. Secondly, models must possess compositional generalization ability to piece together different concept combinations. CommonGen is an effective benchmark for constrained text generation, as its task formulation and evaluation methodology are rather broadly applicable. This is also an advantageous moment to investigate commonsense reasoning capabilities of models, which has received increasing attention through works like COMET \cite{bosselut-etal-2019-comet}.

We experiment on different sizes of BART \cite{lewis-etal-2020-bart} and T5 \cite{JMLR:v21:20-074}, SOTA language generation Transformer models. An initial qualitative analysis (\S\ref{sec:initial_qualitative_analysis}) of baseline generations show several issues related to commonsense, specificity, and fluency. We hypothesize that these issues can be addressed through using images and their captions (\S\ref{sec:initial_image_analysis}). Images representing everyday scenarios are quite commonplace, and are typically logical and grounded in commonsense. Further, image captioning models can normally produce decent captions for everyday images, which can be used to guide the final generation.

%For concept set augmentation, we try two methods for selecting augmented concepts from the train-time human references: extracted keywords, and words with the highest attention. For phrase recombination, we try two methods for recombining the phrases extracted from the baseline models' outputs: mask infilling of text between the phrases, and training phrase-to-text generation models to convert the phrases back into full sentences. \sy{maybe this paragraph is not necessary in the intro}

%Through extensive automatic and human evaluations of our approaches, we show that SAPPHIRE methods noticeably improve model performance on CommonGen across various metrics and aspects of the generated text. An in-depth qualitative analysis illustrates that they effectively address many issues of the baseline model generations, including lack of commonsense, insufficient detail and specificity, and poor fluency. 
%We also demonstrate that they have potential for further exploration and application to general constrained text generation and NLG tasks. \sy{say this last sentence or nah?}

Expounding on this, we use a pretrained image captioning model on MSCOCO captions \cite{lin2015microsoft} to caption the top retrieved images for each concept set (\S\ref{sec:image_retrieval_method},\ref{sec:image_captioning_method}). We use these captions as additional information to augment inputs to our generation models (\S\ref{sec:caption_selection_input_augmentation_method}). Extensive evaluation (\S\ref{sec:results_and_analysis}) demonstrates that VisCTG improves model performance while addressing baseline inadequacies with regards to commonsense, specificity, and fluency.

%methods noticeably improve model performance on CommonGen across various metrics and aspects of the generated text. An in-depth qualitative analysis illustrates that they effectively address many issues of the baseline model generations, including lack of commonsense, insufficient detail and specificity, and poor fluency.

%\sy{Graham's suggestions about framing the paper, maybe discuss data-to-text NLG, keywords-to-text and broader constrained sentence generation, etc.}
%\sy{List of key contributions similar to NAREOR paper}
%\vg{Do we need the typical top right diagram?}
%\sy{see google doc for more discussion on this diagram}
%\sy{Note that we will release all code and data upon acceptance.}
